Multidimensional beyond worst-case and almost-sure problems for mean-payoff objectives

The beyond worst-case threshold problem (BWC), recently introduced by Bruy\`ere et al., asks given a quantitative game graph for the synthesis of a strategy that i) enforces some minimal level of performance against any adversary, and ii) achieves a good expectation against a stochastic model of the adversary. They solved the BWC problem for finite-memory strategies and unidimensional mean-payoff objectives and they showed membership of the problem in NP$\cap$coNP. They also noted that infinite-memory strategies are more powerful than finite-memory ones, but the respective threshold problem was left open. We extend these results in several directions. First, we consider multidimensional mean-payoff objectives. Second, we study both finite-memory and infinite-memory strategies. We show that the multidimensional BWC problem is coNP-complete in both cases. Third, in the special case when the worst-case objective is unidimensional (but the expectation objective is still multidimensional) we show that the complexity decreases to NP$\cap$coNP. This solves the infinite-memory threshold problem left open by Bruy\`ere et al., and this complexity cannot be improved without improving the currently known complexity of classical mean-payoff games. Finally, we introduce a natural relaxation of the BWC problem, the beyond almost-sure threshold problem (BAS), which asks for the synthesis of a strategy that ensures some minimal level of performance with probability one and a good expectation against the stochastic model of the adversary. We show that the multidimensional BAS threshold problem is solvable in P.

==> expectation.tex <==

\section{Expected-value achievable solutions and synthesis inside an EC}



==> fig_losing_EC.tex <==

\begin{figure}
	\begin{center}
		\footnotesize
		\begin{tikzpicture}

			\node[playerstate, initial] (s) [] {$s$};
			\node[randomstate] (t) [right = 1.5cm of s] {$t$};
			\node[playerstate] (s') [below = 1.2cm of s] {$s'$};
		
			\path[->] (s) edge node [above] {$(0, 0)$} (t);
			\path[->] (s) edge node [left] {$(0, 0)$} (s');

			\path[->] (t) edge [bend right = 45] node [above] {$\frac 1 2, (-10, 0)$} (s);
			\path[->] (t) edge [bend left = 45] node [below] {$\frac 1 2, (10, 20)$} (s);
		
			\path[->] (s') edge [loop below] node {$(0, 0)$} ();
		
		\end{tikzpicture}
	\end{center}
	Controller can achieve expected mean payoff $\vec\nu := (0, 5)$ by always going to $t$,
	and guarantee worst-case mean payoff $(0, 0)$ by going to $s'$.
	Notice that the expectation and worst-case thresholds are both $0$ in the first component.
	When Controller plays according to $f^{exp}$ to achieve expected mean payoff $\nu$,
	the total payoff in the first component goes below $-N$ almost surely for any $N \in \N$.
	%
	Therefore, any switching rule looking at the total payoff will eventually pick $f^{wc}$ almost surely,
	which implies that the expectation would be $(0, 0) \not\geq \vec\nu$.
	Therefore, one needs to do something else,
	like looking at the current mean payoff.
	
	\caption{Example of losing EC where it does not suffice to monitor the total payoff to decide when to switch to the worst-case strategy $f^{wc}$. This is due to the fact that the expectation $\vec\nu$ is zero in the first component.}
%	\label{fig:weakly_winning}	
\end{figure}

\begin{figure}
	\begin{center}
		\footnotesize
		\begin{tikzpicture}

			\node[playerstate, initial] (s0) [] {$s_0$};
			\node[randomstate] (t0) [below = 1.2cm of s0] {$t_0$};
		
			\node[playerstate] (s1) [right = 4cm of s0] {$s_1$};
			\node[randomstate] (t1) [below = 1.2cm of s1] {$t_1$};

			\node[playerstate] (s2) [right = 1.5cm of s1] {$s_2$};
		
			\path[->] (s0) edge node [right] {$(0, 0)$} (t0);
			\path[->] (s0) edge [bend left = 30] node [above] {$(-1, -1)$} (s1);

			\path[->] (t0) edge [bend left = 60] node [left] {$\frac 1 2, (20, 0)$} (s0);
			\path[->] (t0) edge [bend right = 75] node [right] {$\frac 1 2, (0, -4)$} (s0);

			\path[->] (s1) edge node [right] {$(0, 0)$} (t1);
			\path[->] (s1) edge node [below] {$(-1, -1)$} (s0);
			\path[->] (s1) edge node [above] {$(0, 0)$} (s2);

			\path[->] (t1) edge [bend left = 60] node [left] {$\frac 1 2, (0, 20)$} (s1);
			\path[->] (t1) edge [bend right = 75] node [right] {$\frac 1 2, (-4, 0)$} (s1);
		
			\path[->] (s2) edge [loop above] node {$(0, 0)$} ();
		
		\end{tikzpicture}
	\end{center}
	
	In the first component $C_0 := \set{s_0, t_0}$ the expected mean payoff is $\nu_0 = (5, -1)$,
	and in the second component $C_1 := \set {s_1, t_1}$ it is $\nu_1 = (-1, 5)$.
	Thus, the vector $\nu := (2, 2)$ is achievable in expectation.
	However, the EC $C_0 \cup C_1$ is losing since it is not possible to guarantee worst-case mean payoff $\geq (0, 0)$
	without leaving it and going to $s_2$.
	
	Note that playing according to a (finite-memory, randomized) strategy $f^{exp}$
	that chooses whether to stay in $C_0$ or in $C_1$ with equal probability is losing for the BWC objective,
	since saying forever in $C_i$ will violate the worst-case objective almost surely
	(since $\nu_i$ has a negative component),
	which implies that such a $f^{exp}$ is almost surely replaced by $f^{wc}$.
	
	Therefore, we need to use $f^{exp}$ which cycles between $C_0$ and $C_1$,
	but this requires infinite memory...! Problem!
	(Infinite memory is a problem because in the resulting infinite Markov chain
	it is difficult to argue about the probability that we are close to the expected mean payoff.)
	
	Note: This can be addressed by using a sequence of finite-memory strategies inducing unichains
	and providing better and better approximations to the expectation.
	
	\caption{Example of losing EC where one cannot win if using a $f^{exp}$ which induces two different SCCs.}
%	\label{fig:weakly_winning}	
\end{figure}


==> fig_system_V.tex <==


\begin{figure}
	Assume that the starting state $s_0$ belongs to Controller.
	%
	\begin{align}
		1_{s_0}(s) + \sum_{(r, s) \in E} y_{rs} &= \sum_{(s, t) \in E} y_{st} + y_s
			&& \forall s \in S
		\label{eq:V:y:flow}
		\\
		y_{st} &= R(s)(t) \cdot ( \!\! \sum_{(r, s) \in E} \!\!\!\! y_{rs} - y_s)
			&& \forall (s, t) \in E \textrm{ with } s \in S^R
		\label{eq:V:y:random}
		\\
		\sum_{s \in S} y_s &= 1
		\label{eq:V:y:sum}
		\\
		\sum_{s \in U} y_s &= \sum_{(r, s) \in E\cap U \times U} x_{rs}
		 	&& \forall \textrm{ MEC } U
		\label{eq:V:x:y}
		\\
		\sum_{(r, s) \in E} x_{rs} &= \sum_{(s, t) \in E} x_{st}
			&& \forall s \in S
		\label{eq:V:x:flow}
		\\
		x_{st} &= R(s)(t) \cdot \sum_{(r, s) \in E} x_{rs}
			&& \forall (s, t) \in E \textrm{ with } s \in S^R
		\label{eq:V:x:random}
		\\
		\sum_{(s, t) \in E} x_{st} \cdot w(s, t)[i] & > \vec \nu[i] 
			&& \forall (1 \leq i \leq n)
		\label{eq:V:MP:global}
		\\
		\sum_{(s, t) \in E\cap U \times U} \!\!\!\!\!\!\!\! x_{st} \cdot w(s, t)[i] & > 0
			&& \forall \textrm{ MEC } U, 1 \leq i \leq n
		\label{eq:V:MP:local}
	\end{align}
	
	\caption{Linear system $V$ for the beyond almost-sure threshold problem.}
	\label{fig:BAS:system}
\end{figure}

